Using Deep Reinforcement Learning to Learn High-Level Policies on the ATRIAS Biped

Learning controllers for bipedal robots is a challenging problem, often requiring expert knowledge and extensive tuning of parameters that vary in different situations. Recently, deep reinforcement learning has shown promise at automatically learning controllers for complex systems in simulation. This has been followed by a push towards learning controllers that can be transferred between simulation and hardware, primarily with the use of domain randomization. However, domain randomization can make the problem of finding stable controllers even more challenging, especially for underactuated bipedal robots. In this work, we explore whether policies learned in simulation can be transferred to hardware with the use of high-fidelity simulators and structured controllers. We learn a neural network policy which is a part of a more structured controller. While the neural network is learned in simulation, the rest of the controller stays fixed, and can be tuned by the expert as needed. We show that using this approach can greatly speed up the rate of learning in simulation, as well as enable transfer of policies between simulation and hardware. We present our results on an ATRIAS robot and explore the effect of action spaces and cost functions on the rate of transfer between simulation and hardware. Our results show that structured policies can indeed be learned in simulation and implemented on hardware successfully. This has several advantages, as the structure preserves the intuitive nature of the policy, and the neural network improves the performance of the hand-designed policy. In this way, we propose a way of using neural networks to improve expert designed controllers, while maintaining ease of understanding.

==> related_work.tex <==
\section{RELATED WORK}
In recent years, several different deep reinforcement learning approaches have been proposed for continuous tasks. The leading contender is 'vanilla' policy gradient method \cite{mnih2016asynchronous}, this method is easy to implement but have poor data efficiency and robustness. Trust region policy optimization (TRPO) \cite{schulman2015trust} adds a constraint on the size of the policy update so that TRPO is easier to converge to good result but it's relatively complicated to implement. Proximal Policy Optimization \cite{schulman2017proximal}\cite{heess2017emergence} using first-order optimization which is simpler to implement than TRPO while being stable and data efficient. Deep Deterministic Policy Gradient \cite{lillicrap2015continuous} is based on the Deterministic Policy Gradient(DPG)  \cite{silver2014deterministic} algorithm and Deep Q Network(DQN) \cite{mnih2013playing}, in practice, DDPG is not so stable and some researchers combined DDPG with a demo augmented objective to enhance its stability\cite{rajeswaran2017learning}. 

Some work have incorporating demonstrations with reinforcement learning for better performance. Dynamic movement primitives method \cite{kober2009learning}\cite{theodorou2010reinforcement} combines demonstration with reinforcement learning but this method limits to function representation. Using motion capture data as demonstrations \cite{merel2017learning}, has been used to initialize policies via behavior cloning. Also, demonstrations can be used to pre-train a Q-function by minimizing TD error \cite{sendonaris2017learning}. Some researchers used demonstrations to guide exploration through incorporating demonstration with reward function shaping \cite{subramanian2016exploration} \cite{taylor2011integrating}. Demonstration can also be used to find cost function which is known as inverse reinforcement learning \cite{ng2000algorithms}\cite{russell1998learning}.

As mentioned above, there are many methods that can be used for control task.  Using these methods, agents can develop impressive dynamic motor skills \cite{wang2017robust}\cite{heess2017emergence}\cite{peng2016terrain}.  However, due to the high simple complexity of these methods as well as other physical limitations, many of the capability demonstrated in simulation cannot be replicated on hardware. There are very few algorithms that has been demonstrated that can training policies directly on hardware such as Guided Policy Search \cite{levine2013guided}. Some researchers seek out way to tune parameters to overcome the difference between simulation environment and physical world. One of the method is using Bayesian Optimization \cite{antonova2017deep}. Yet this method cannot tune be used for tuning deep neural network. In sum, successful examples of training policies directly on hardware are limited to relatively restrictive domain so far \cite{peng2017sim}.
